ACME: A Multi-Cultural, Multi-Embodiment Social-Navigation Dataset

Understanding how robots and humans move in shared spaces is essential for designing effective social robot navigation policies and predicting human behavior. However, existing datasets often lack the diversity needed to capture differences in culture, geography, and human-robot interaction-factors that strongly shape appropriate social behavior. To address this gap, we introduce ACME: A Cross-cultural, Multi-Embodiment dataset for social navigation. A large-scale data collection effort across 8 sites in 5 countries, using 7 robot embodiments, ACME is a large and diverse multi-modal dataset aimed at advancing social navigation research, providing 29.35 hours of onboard robot data and 43.5 hours of overhead pedestrian tracking data. Unlike prior datasets, it focuses on capturing goal-driven social navigation behavior in complex social scenarios with explicit robot-crowd interaction through robot speech. To facilitate learning navigation policies and predicting pedestrian trajectories, ACME provides 3D and 2D scene features, odometry, interaction information, and human-annotated pedestrian trajectory labels. We make ACME easy to use by providing both human-readable data for each sensor modality as well as raw binary data. Our qualitative and quantitative analyses show that our dataset captures more challenging scenarios and a broader distribution of pedestrian behavior than previous datasets.

==> default_template.tex <==












\section{The article header information}
The heading for any file using \textsf{\journalclass} is shown in
Figure~\ref{F1}. You must select options for the trim/text area and
the reference style of the journal you are submitting to.
The choice of \verb+options+ are listed in Table~\ref{T1}.

\begin{table}[h]
\small\sf\centering
\caption{The choice of options.\label{T1}}
\begin{tabular}{lll}
\toprule
Option&Trim and font size&Columns\\
\midrule
\texttt{shortAfour}& 210 $\times$ 280 mm, 10pt& Double column\\
\texttt{Afour} &210 $\times$ 297 mm, 10pt& Double column\\
\texttt{MCfour} &189 $\times$ 246 mm, 10pt& Double column\\
\texttt{PCfour} &170 $\times$ 242 mm, 10pt& Double column\\
\texttt{Royal} &156 $\times$ 234 mm, 10pt& Single column\\
\texttt{Crown} &7.25 $\times$ 9.5 in, 10pt&Single column\\
\texttt{Review} & 156 $\times$ 234 mm, 12pt & Single column\\
\bottomrule
\end{tabular}\\[10pt]
\begin{tabular}{ll}
\toprule
Option&Reference style\\
\midrule
\texttt{sageh}&SAGE Harvard style (author-year)\\
\texttt{sagev}&SAGE Vancouver style (superscript numbers)\\
\texttt{sageapa}&APA style (author-year)\\
\bottomrule
\end{tabular}
\end{table}

For example, if your journal is short A4 sized, uses Times fonts and has Harvard style references then you would need\\
{\small\verb+\documentclass[ShortAfour,times,sageh]{sagej}+}

Most \textit{SAGE} journals are published using Times fonts but if for any reason you have a problem using Times you can
easily resort to Computer Modern fonts by removing the
\verb"times" option.

\subsection{`Review' option}
Some journals (for example, \emph{Journal of the Society for Clinical Trials}) require that
papers are set single column and with a larger font size to help with the review process.
If this is a requirement for the journal that you are submitting to, just add the \verb+Review+ option to the \verb+\documenclass[]{sagej}+ line.

\subsection{Remarks}
\begin{enumerate}
\item[(i)] In \verb"\runninghead" use `\textit{et~al.}' if there
are three or more authors.

\item[(ii)] For multiple author papers please note the use of \verb"\affilnum" to
link names and affiliations. The corresponding author details need to be included using the
\verb+\corrauth+ and \verb+\email+ commands.

\item[(iii)] For submitting a double-spaced manuscript, add
\verb"doublespace" as an option to the documentclass line.

\item[(iv)] The abstract should be capable of standing by itself,
in the absence of the body of the article and of the bibliography.
Therefore, it must not contain any reference citations.

\item[(v)] Keywords are separated by commas.

\item[(vi)] If you are submitting to a \textit{SAGE} journal that requires numbered sections (for example, IJRR), please add the command
  \verb+\setcounter{secnumdepth}{3}+ just above the \verb+\begin{document}+ line.

\end{enumerate}


\section{The body of the article}

\subsection{Mathematics} \textsf{\journalclass} makes the full
functionality of \AmS\/\TeX\ available. We encourage the use of
the \verb"align", \verb"gather" and \verb"multline" environments
for displayed mathematics. \textsf{amsthm} is used for setting
theorem-like and proof environments. The usual \verb"\newtheorem"
command needs to be used to set up the environments for your
particular document.

\subsection{Figures and tables} \textsf{\journalclass} includes the
\textsf{graphicx} package for handling figures.

Figures are called in as follows:
\begin{verbatim}
\begin{figure}
\centering
\includegraphics{<figure name>}
\caption{<Figure caption>}
\end{figure}
\end{verbatim}

For further details on how to size figures, etc., with the
\textsf{graphicx} package see, for example, \cite{R1}
or \cite{R3}.

The standard coding for a table is shown in Figure~\ref{F2}.

\begin{figure}
\setlength{\fboxsep}{0pt}%
\setlength{\fboxrule}{0pt}%
\begin{center}
\begin{boxedverbatim}
\begin{table}
\small\sf\centering
\caption{<Table caption.>}
\begin{tabular}{<table alignment>}
\toprule
<column headings>\\
\midrule
<table entries
(separated by & as usual)>\\
<table entries>\\
.
.
.\\
\bottomrule
\end{tabular}
\end{table}
\end{boxedverbatim}
\end{center}
\caption{Example table layout.\label{F2}}
\end{figure}

\subsection{Cross-referencing}
The use of the \LaTeX\ cross-reference system
for figures, tables, equations, etc., is encouraged
(using \verb"\ref{<name>}" and \verb"\label{<name>}").

\subsection{End of paper special sections}
Depending on the requirements of the journal that you are submitting to,
there are macros defined to typeset various special sections.

The commands available are:
\begin{verbatim}
\begin{acks}
To typeset an
  "Acknowledgements" section.
\end{acks}
\end{verbatim}

\begin{verbatim}
\begin{biog}
To typeset an
  "Author biography" section.
\end{biog}
\end{verbatim}

\begin{verbatim}
\begin{biogs}
To typeset an
  "Author Biographies" section.
\end{biogs}
\end{verbatim}


\begin{verbatim}
\begin{dci}
To typeset a "Declaration of
  conflicting interests" section.
\end{dci}
\end{verbatim}

\begin{verbatim}
\begin{funding}
To typeset a "Funding" section.
\end{funding}
\end{verbatim}

\begin{verbatim}
\begin{sm}
To typeset a
  "Supplemental material" section.
\end{sm}
\end{verbatim}

\subsection{Endnotes}
Most \textit{SAGE} journals use endnotes rather than footnotes, so any notes should be coded as \verb+\endnote{<Text>}+.
Place the command \verb+\theendnotes+ just above the Reference section to typeset the endnotes.

To avoid any confusion for papers that use Vancouver style references,  footnotes/endnotes should be edited into the text.

\subsection{References}
Please note that the files \textsf{SageH.bst} and \textsf{SageV.bst} are included with the class file
for those authors using \BibTeX.
The files work in a completely standard way, and you just need to uncomment one of the lines in the below example depending on what style you require:
\begin{verbatim}
\bibliography{<YourBibfile.bib>}
\end{verbatim}
and remember to add the relevant option to the \verb+\documentclass[]{sagej}+ line as listed in Table~\ref{T1}. 


\section{Copyright statement}
Please  be  aware that the use of  this \LaTeXe\ class file is
governed by the following conditions.

\subsection{Copyright}
Copyright \copyright\ \volumeyear\ SAGE Publications Ltd,
1 Oliver's Yard, 55 City Road, London, EC1Y~1SP, UK. All
rights reserved.

\subsection{Rules of use}
This class file is made available for use by authors who wish to
prepare an article for publication in a \textit{SAGE Publications} journal.
The user may not exploit any
part of the class file commercially.

This class file is provided on an \textit{as is}  basis, without
warranties of any kind, either express or implied, including but
not limited to warranties of title, or implied  warranties of
merchantablility or fitness for a particular purpose. There will
be no duty on the author[s] of the software or SAGE Publications Ltd
to correct any errors or defects in the software. Any
statutory  rights you may have remain unaffected by your
acceptance of these rules of use.

\begin{acks}
This class file was developed by Sunrise Setting Ltd,
Brixham, Devon, UK.\\
Website: \url{http://www.sunrise-setting.co.uk}
\end{acks}

\begin{thebibliography}{99}
\bibitem[Kopka and Daly(2003)]{R1}
Kopka~H and Daly~PW (2003) \textit{A Guide to \LaTeX}, 4th~edn.
Addison-Wesley.

\bibitem[Lamport(1994)]{R2}
Lamport~L (1994) \textit{\LaTeX: a Document Preparation System},
2nd~edn. Addison-Wesley.

\bibitem[Mittelbach and Goossens(2004)]{R3}
Mittelbach~F and Goossens~M (2004) \textit{The \LaTeX\ Companion},
2nd~edn. Addison-Wesley.

\end{thebibliography}


==> novelty_statement.tex <==
\section{Novelty Statement}
ACME introduces the first large-scale dataset and benchmark for social navigation spanning multiple cultures and robot embodiments: 8 collection teams across 5 countries using 7 robot platforms. It uniquely captures goal-driven robot–crowd interactions, including robot speech, synchronized multimodal onboard and bird’s-eye-view data, human-verified pedestrian trajectories, scenario tags, and benchmarks for navigation and trajectory prediction. This directly advances IJRR’s scope by enabling robust, context- and embodiment-aware robot navigation in human environments.

